FocusMAE: Gallbladder Cancer Detection from Ultrasound Videos with Focused Masked Autoencoders

In recent years, automated Gallbladder Cancer (GBC) detection has gained the attention of researchers. Current state-of-the-art (SOTA) methodologies relying on ultrasound sonography (US) images exhibit limited generalization, emphasizing the need for transformative approaches. We observe that individual US frames may lack sufficient information to capture disease manifestation. This study advocates for a paradigm shift towards video-based GBC detection, leveraging the inherent advantages of spatiotemporal representations. Employing the Masked Autoencoder (MAE) for representation learning, we address shortcomings in conventional image-based methods. We propose a novel design called FocusMAE to systematically bias the selection of masking tokens from high-information regions, fostering a more refined representation of malignancy. Additionally, we contribute the most extensive US video dataset for GBC detection. We also note that, this is the first study on US video-based GBC detection. We validate the proposed methods on the curated dataset, and report a new state-of-the-art (SOTA) accuracy of 96.4% for the GBC detection problem, against an accuracy of 84% by current Image-based SOTA - GBCNet, and RadFormer, and 94.7% by Video-based SOTA - AdaMAE. We further demonstrate the generality of the proposed FocusMAE on a public CT-based Covid detection dataset, reporting an improvement in accuracy by 3.3% over current baselines. The source code and pretrained models are available at: https://gbc-iitd.github.io/focusmae

==> sections/table-supple-hyper.tex <==
\begin{table*}[ht]
	\centering
    \small
	%\resizebox{ \linewidth}{!}{%
	\begin{tabular}{cccccccc}
		\toprule
		\multirow{3}{*}{\textbf{Masking Ratio}} & \multirow{3}{*}{\textbf{Decoder Depth}} & \multicolumn{6}{c}{\textbf{Loss}} \\
        & & \multicolumn{3}{c}{\textbf{MSE}} & \multicolumn{3}{c}{\textbf{L1}} \\
        & & Acc. & Spec. & Sens. & Acc. & Spec. & Sens. \\
        %& {\textbf{Time/Frame (ms)}}\\
		\midrule
		%
        \multirow{4}{*}{0.6}
		& 4  & 0.538$\pm$0.443 & 0.808$\pm $0.123& 0.910$\pm$0.117 & 0.943$\pm$0.065 
         & 0.910$\pm$0.117 & 0.938$\pm$0.076 \\
  
        & 6 & 0.945$\pm$0.071 & 0.910$\pm$0.117 & 1.000$\pm$0.000 & 0.943$\pm$0.065& 0.910$\pm$0.117& 0.938$\pm$0.076  \\
        
        & 8 & 0.942$\pm$0.066 & 0.910$\pm$0.117 & 0.938$\pm$0.076& 0.943$\pm$0.065 & 0.910$\pm$0.117 & 0.938$\pm$0.076  \\
        
        & 10 & 0.749$\pm$0.144 & 0.910$\pm$0.117 & 0.600$\pm$0.490  & 0.943$\pm$0.065 & 0.910$\pm$0.117 & 0.938$\pm$0.076  \\
		%
        \midrule 
        %
		\multirow{4}{*}{0.8}
		& 4 & 0.940$\pm$0.066  & 0.910$\pm$0.117& 0.938$\pm$0.076 & 0.86$\pm$0.124 & 0.699$\pm$0.371 & 0.910$\pm$0.117 \\
        & 6 & 0.942$\pm$0.065  & 0.910$\pm$0.117 & 0.938$\pm$0.076 & 0.943$\pm$0.065 & 1.000$\pm$0.000 & 0.938$\pm$0.076 \\
        & 8 & 0.942$\pm$0.066 & 0.910$\pm$0.117 & 0.938$\pm$0.076 & 0.978$\pm$0.027 & 1.000$\pm$0.000 & 0.938$\pm$0.076\\
        & 10 & 0.952$\pm$0.070 & 0.910$\pm$0.117 & 0.967$\pm$0.067 & 0.943$\pm$0.065 & 0.910$\pm$0.117 & 0.938$\pm$0.076 \\
		%
        \midrule 
        %
        \multirow{4}{*}{0.95}
		& 4 & 0.810$\pm$0.124 &0.910$\pm$0.117& 0.538$\pm$0.443 & 0.943$\pm$0.065 &0.910$\pm$0.117 & 0.938$\pm$0.076 \\
        & 6 & 0.943$\pm$0.065 & 0.910$\pm$0.117 & 0.938$\pm$0.076& 0.943$\pm$0.065 & 0.910$\pm$0.117 & 0.938$\pm$0.076 \\
        & 8 & 0.811$\pm$0.122&0.910$\pm$0.117 & 0.538$\pm$0.443 & 0.943$\pm$0.065 & 0.910$\pm$0.117 & 0.938$\pm$0.076 \\
        & 10 & 0.964$\pm$0.072 & 0.910$\pm$0.117 & 1.000$\pm$0.000 & 0.943$\pm$0.065& 0.910$\pm$0.117 & 0.938$\pm$0.076 \\
		%
  %       \midrule 
  %       %
  %       \multirow{4}{*}{1}
		% & 4 & 0.966$\pm$0.028 & 1.000$\pm$0.000 & 0.909$\pm$0.074 & 0.965$\pm$0.071 & 0.910$\pm$0.117 & 1.000$\pm$0.000 \\
  %       & 6 & 0.943$\pm$0.065 & 0.910$\pm$0.117& 0.938$\pm$0.076 &0.943$\pm$0.065 &1.000$\pm$0.000 &0.938$\pm$0.076  \\
  %       & 8 & 0.943$\pm$0.065 & 0.910$\pm$0.117 & 0.938$\pm$0.076 & 0.943$\pm$0.065 &1.000$\pm$0.000 &0.938$\pm$0.076  \\
  %       & 10 & 0.966$\pm$0.028 & 1.000$\pm$0.000 & 0.91$\pm$0.074 & 0.943$\pm$0.065 &1.000$\pm$0.000 &0.938$\pm$0.076 \\
		\bottomrule
	\end{tabular}
	%}
	\caption{Hyperparameter tuning. We vary the Masking ratio, Decoder depth, and the loss function for a grid search. We report the 5-fold cross-validation (Mean$\pm$SD) accuracy, specificity, and sensitivity for \myarch in detecting GBC from the US. 
    }
	\label{tab:hyperparam_supp}
\end{table*}

